Scaling limit of subcritical contact process

In this paper we describe the subcritical contact process on $\Z^d$ for large times, starting with all sites infected. The configuration is described in terms of the macroscopic locations of infected regions in space and the relative positions of infected sites in each such region.

==> figures/fig_pyramid.tex <==
\begin{tikzpicture}[scale=0.7]

% projection 3d -> 2D
\def\point(#1,#2,#3){(#1+0.3*#2,#3+0.4*#2)}
% le reseau Z^2 en fond
\foreach \x in {-6,-5, -4, -3, -2, -1, 0, 1, 2, 3, 4, 5}
  \foreach \y in {-3, -2, -1, 0, 1, 2, 3,4}
    \draw[fill] \point(\x, \y, 0) circle[radius=1pt];

% code d'un cube #1 hauteur de depart #2 rayon
\def\base(#1,#2){%
\draw[fill=white] \point(-#2,-#2,#1) -- %
      \point(-#2,#2,#1) -- %
      \point(#2,#2,#1) -- %
      \point(#2,-#2,#1) -- %
      cycle; %
\draw[fill=white] \point(-#2,#2,#1) -- %
      \point(#2,#2,#1) -- %
      \point(#2,#2,#1+1) -- %
      \point(-#2,#2,#1+1) -- %
      cycle; %
\draw[fill=white] \point(-#2,-#2,#1) -- %
      \point(-#2,#2,#1) -- %
      \point(-#2,#2,#1+1) -- %
      \point(-#2,-#2,#1+1) -- %
      cycle; %
\draw[fill=white] \point(#2,-#2,#1) -- %
      \point(#2,#2,#1) -- %
      \point(#2,#2,#1+1) -- %
      \point(#2,-#2,#1+1) -- %
      cycle; %
\draw[fill=white] \point(#2,-#2,#1) -- %
      \point(-#2,-#2,#1) -- %
      \point(-#2,-#2,#1+1) -- %
      \point(#2,-#2,#1+1) -- %
      cycle; %
\draw[fill=white] \point(-#2,-#2,#1+1) -- %
      \point(-#2,#2,#1+1) -- %
      \point(#2,#2,#1+1) -- %
      \point(#2,-#2,#1+1) -- %
      cycle; %
}

% et j'en supperpose 4
\base(0, 3);
\base(1, 2);
\base(2, 1);
\base(3, 0);
%legendes
\draw[arrows=<->] \point(-3, -3, -0.3) -- \point(3, -3, -0.3);
\draw \point(0,-3, -0.3) node [below] {$2\lfloor4\beta\sqrt{t}\rfloor$};

\draw[arrows=<->] \point(-3.3, -3, 0) -- \point(-3.3, -3, 1);
\draw[fill,white] \point(-4, -2, 0) circle[radius=2pt];
\draw \point(-3.3, -3, 0.5) node[left] {$\frac{1}{4\beta}$};

\draw \point(6, -1, 0) -- \point(8, -1, 0) -- \point(8, 1, 0) -- \point(6, 1, 0) -- cycle;
\draw \point(8,-1,0) node [left, above] {$\mathbb{Z}^d$};

\draw[arrows=-latex] \point(7,0,0) -- \point(7,0,1.5);
\draw \point(7,0,1.5) node [right] {$\mathbb{R^+}$};
\end{tikzpicture}
